Tests of hadronic interactions with measurements by Pierre Auger Observatory

The hybrid design of the Pierre Auger Observatory allows for the measurement of a number of properties of extensive air showers initiated by ultra-high energy cosmic rays. By comparing these measurements to predictions from air shower simulations, it is possible to both infer the cosmic ray's mass composition and test hadronic interactions beyond the energies reached by accelerators. In this paper, we will present a compilation of results of air shower measurements by Pierre Auger Observatory which are sensitive to the properties of hadronic interactions and can be used to constrain the hadronic interaction models. The inconsistencies found between the interpretation of different observables with regard to primary composition and between their measurements and simulations show that none of the currently used hadronic interaction models can provide a proper description of air showers and, in particular, of the muon production.

==> BeamerUtil.tex <==
%%LOCAL COLORS
\definecolor{ThisBlue}{RGB}{50,50,168}
\definecolor{ThisRed}{RGB}{225,0,0}
\definecolor{ThisGray}{RGB}{150,150,150}


%%FUNCTIONS
\def\Put(#1,#2)#3{\leavevmode\makebox(0,0){\put(#1,#2){#3}}}

\newcommand{\hsp}[1]{\hspace*{#1cm}}
\newcommand{\vsp}[1]{\vspace*{#1cm}}

\newcommand{\reference}[1]{\textcolor{ThisGray}{#1}}
\newcommand{\arxiv}[1]{\href{https://arxiv.org/abs/#1}{\texttt{arXiv:#1}}}


%%BULLETS
\newcommand{\myarrow}{\textcolor{ThisRed}{\raisebox{0.4ex}[-0.4ex]{\tiny$\blacktriangleright$\xspace}}}
\newcommand{\mybullet}{\textcolor{ThisBlue}{\footnotesize $\bullet$}\xspace}  


%%ENVIROMENTS
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bcols}{\begin{columns}}
\newcommand{\ecols}{\end{columns}}
\newcommand{\bcol}{\begin{column}}
\newcommand{\ecol}{\end{column}}
\newcommand{\bop}{\begin{overpic}}
\newcommand{\eop}{\end{overpic}}
\newcommand{\bbe}{\begin{equation*}}
\newcommand{\eee}{\end{equation*}}
\newcommand{\btikz}{\begin{tikzpicture}}
\newcommand{\etikz}{\end{tikzpicture}}

\newcommand{\bbox}[1]{\begin{tcolorbox}[colframe=#1,colback=white,left=0.2pt,right=0.2pt,top=0.5pt,bottom=0.5pt]}
\newcommand{\ebox}{\end{tcolorbox}}

